Abstract independence relations in neostability theory

We develop a framework, in the style of Adler, for interpreting the notion of "witnessing" that has appeared (usually as a variant of Kim's Lemma) in different areas of neostability theory as a binary relation between abstract independence relations. This involves extending the relativisations of Kim-independence and Conant-independence due to Mutchnik to arbitrary independence relations. After developing this framework, we show that several results from simplicity, $\text{NTP}_2$, $\text{NSOP}_1$, and beyond follow as instances of general theorems for abstract independence relations. In particular, we prove the equivalence between witnessing and symmetry and the implications from this notion to chain local character and the weak independence theorem, and recover some partial converses. Finally, we use this framework to prove a dichotomy between $\text{NSOP}_1$ and Kruckman and Ramsey's $\text{BTP}$ that applies to most known $\text{NSOP}_4$ examples in the literature.

==> header.tex <==
%Maths Packages
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{qtree}
\usepackage{array}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{cancel}
\usepackage{tikz}
\usepackage{comment}
\usepackage{theoremref}

% Show labels (for easier references)
% To turn off the showing of labels add the final option, like so:
%\usepackage[inline,final]{showlabels}
\usepackage[inline,final]{showlabels}
\showlabels{thlabel}

%Plot
\usepackage{pgfplots}
\usepgfplotslibrary{polar}
\pgfplotsset{width=10cm,compat=1.9}

%Size
\usepackage{geometry}
%\geometry{margin = 1.4in} %For normal, 12pt size
\geometry{margin = 1.75in}
\RequirePackage{mdwtab,latexsym,amsmath,amsfonts,ifthen}
\usepgfplotslibrary{external}

%Graphs
\usepackage{tikz}
%\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{cd}

\newcounter{counter}
\newcounter{blop}
\setcounter{blop}{6}

%Mathematical Environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{nonumthm}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{nonumprop}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{nonumcor}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{nonumlemma}{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem*{nonumcon}{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem*{nfact}{Fact}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{nonumdef}{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem*{nonumex}{Example}
\newtheorem*{exercise}{Exercise}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{nonumrem}{Remark}
\newtheorem*{claim}{Claim}
\newtheorem{nclaim}[counter]{Claim}
\newtheorem*{subclaim}{Subclaim}
\newtheorem*{convention}{Convention}
\newtheorem*{notation}{Notation}
\newtheorem*{terminology}{Terminology}
\newtheorem*{discussion}{Discussion}
\newtheorem*{open}{Open question}
\newtheorem*{question}{Question}

% Add to Preamble
\newenvironment{restate}[1]{%
  \begingroup % Localize changes
  \renewcommand{\thetheorem}{\ref{#1}} % Set theorem number to the referenced label
  \begin{theorem}%
}{%
  \end{theorem}%
  \addtocounter{theorem}{-1} % Decrement counter so next theorem in Intro is numbered correctly
  \endgroup
}

% Restate Proposition (uses shared 'theorem' counter)
\newenvironment{restateprop}[1]{%
  \begingroup
  \renewcommand{\thetheorem}{\ref{#1}} % Redefine the shared label formatting
  \begin{proposition}%
}{%
  \end{proposition}%
  \addtocounter{theorem}{-1} % Reset the SHARED counter
  \endgroup
}

% Restate Corollary (uses shared 'theorem' counter)
\newenvironment{restatecor}[1]{%
  \begingroup
  \renewcommand{\thetheorem}{\ref{#1}} % Redefine the shared label formatting
  \begin{corollary}%
}{%
  \end{corollary}%
  \addtocounter{theorem}{-1} % Reset the SHARED counter
  \endgroup
}

\usepackage{graphicx}

%Change label in enumerate
\usepackage[shortlabels]{enumitem}

%Style of subsections
\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{2}%
  \z@{.5\linespacing\@plus.7\linespacing}{-.5em}%
  {\normalfont\bfseries}}
\makeatother

%Change the position of subsection title in table of contents
\setcounter{tocdepth}{1}% to get subsubsections in toc
% \let\oldtocsection=\tocsection
% \let\oldtocsubsection=\tocsubsection
% \let\oldtocsubsubsection=\tocsubsubsection
%\renewcommand{\tocsection}[2]{\hspace{0em}\oldtocsection{#1}{#2}}
%\renewcommand{\tocsubsection}[2]{\hspace{1.8em}\oldtocsubsection{#1}{#2}}
%\renewcommand{\tocsubsubsection}[2]{\hspace{4.4em}\oldtocsubsubsection{#1}{#2}}

\numberwithin{equation}{section}

\usepackage[british]{babel}
\babelhyphenation[british]{i-ma-gi-na-ries}
\babelhyphenation[british]{ho-mo-ge-neous}
\babelhyphenation[british]{amal-ga-ma-tion}
\babelhyphenation[british]{pseudo-fi-nite}

%Number sets
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}

%Arrows
\newcommand{\hooklongrightarrow}{\lhook\joinrel\longrightarrow}

%Caligraphic style
\renewcommand{\l}{\mathcal{L}}
\newcommand{\m}{\mathcal{M}}
\newcommand{\n}{\mathcal{N}}
\newcommand{\meq}{\mathcal{M}^{\text{eq}}}
\renewcommand{\a}{\mathcal{A}}
\renewcommand{\d}{\mathcal{D}}
\newcommand{\cons}{\mathcal{C}}
\newcommand{\rel}{\mathcal{R}}
\newcommand{\func}{\mathcal{F}}
\renewcommand{\u}{\mathcal{U}}

%Algebraic Geometry Notation
\newcommand{\V}{\mathbb{V}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\A}{\mathbb{A}}
\DeclareMathOperator{\Spec}{\textnormal{Spec}} 

%Galois Theory Notation
\newcommand{\Gal}{\textnormal{Gal}}

%Algebra Notation
\newcommand{\Ass}{\textnormal{Ass}}
\newcommand{\Ann}{\textnormal{Ann}}
\newcommand{\Supp}{\textnormal{Supp}}
\newcommand{\p}{\mathfrak{p}}
\newcommand{\q}{\mathfrak{q}}
\renewcommand{\char}{\textnormal{char} \:}

%Theories
\newcommand{\DLO}{\mathsf{DLO}}
\newcommand{\ACF}{\mathsf{ACF}}
\newcommand{\RG}{\mathsf{RG}}
\newcommand{\TFDAG}{\mathsf{TFDAG}}
\newcommand{\ZFC}{\mathsf{ZFC}}
\newcommand{\RCF}{\mathsf{RCF}}
\newcommand{\DCF}{\mathsf{DCF}}

%Normal text in formulas within definition environments
\DeclareMathOperator{\tm}{\textnormal{tm}}
\DeclareMathOperator{\fml}{\textnormal{Fml}}
\DeclareMathOperator{\sen}{\textnormal{Sen}}
\DeclareMathOperator{\vbl}{\textnormal{Vbl}}
\DeclareMathOperator{\fr}{\textnormal{Fr}}
\DeclareMathOperator{\ded}{\textnormal{Ded}}
%\renewcommand{\th}{\textnormal{Th}}
\DeclareMathOperator{\ctm}{\textnormal{ctm}}
\DeclareMathOperator{\tmalg}{\textnormal{TmAlg}}
\DeclareMathOperator{\tp}{\textnormal{tp}}
\DeclareMathOperator{\stp}{\textnormal{stp}}
\DeclareMathOperator{\diag}{\textnormal{Diag}}
\DeclareMathOperator{\eldiag}{\textnormal{Diag}_{\textnormal{el}}}
\newcommand{\acl}{\textnormal{acl}}
\DeclareMathOperator{\dcl}{\textnormal{dcl}}
\DeclareMathOperator{\Def}{\textnormal{Def}}
%\DeclareMathOperator{\lind}{\textnormal{Lind}}
\DeclareMathOperator{\mult}{\textnormal{mult}}
\DeclareMathOperator{\cl}{\textnormal{cl}}
\DeclareMathOperator{\bdd}{\textnormal{bdd}}

%Cool Greek
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}

%Set-theoretic operations
\newcommand{\size}[1]{\lvert #1 \rvert}
\newcommand{\nmodels}{\mathbin{\cancel{\models}} \:}
\newcommand{\equ}{\sim_{\Sigma}}
\newcommand{\Ord}{\textnormal{Ord}}

%Model-theoretic symbols
\def\Ind#1#2{#1\setbox0=\hbox{$#1x$}\kern\wd0\hbox to 0pt{\hss$#1\mid$\hss}
\lower.9\ht0\hbox to 0pt{\hss$#1\smile$\hss}\kern\wd0}

\def\ind{\mathop{\mathpalette\Ind{}}}

\def\notind#1#2{#1\setbox0=\hbox{$#1x$}\kern\wd0
\hbox to 0pt{\mathchardef\nn=12854\hss$#1\nn$\kern1.4\wd0\hss}
\hbox to 0pt{\hss$#1\mid$\hss}\lower.9\ht0 \hbox to 0pt{\hss$#1\smile$\hss}\kern\wd0}

\def\nind{\mathop{\mathpalette\notind{}}}

\newcommand{\forkindep}[1][]{%
  \mathrel{
    \mathop{
      \vcenter{
        \hbox{\oalign{\noalign{\kern-.3ex}\hfil$\vert$\hfil\cr
              \noalign{\kern-.7ex}
              $\smile$\cr\noalign{\kern-.3ex}}}
      }
    }\displaylimits_{#1}
  }
}
\renewcommand{\H}{\mathcal{H}}
%\newcommand{\f}{\mathcal{F}}
\newcommand{\RM}{\textnormal{RM}}
\newcommand{\U}{\textnormal{U}}
\newcommand{\SU}{\textnormal{SU}}
\newcommand{\RC}{\textnormal{RC}}
\renewcommand{\r}{\textnormal{R}}
\newcommand{\D}{\textnormal{D}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\eq}{\textnormal{eq}}
\newcommand{\heq}{\textnormal{heq}}
\newcommand{\Cb}{\textnormal{Cb}}
\newcommand{\nc}{\textnormal{nc}}
\newcommand{\ls}{\textnormal{Ls}}
\renewcommand{\i}{\textnormal{i}}
\newcommand{\f}{\textnormal{f}}

%General shortcuts
\newcommand{\bx}{\bar{x}}
\newcommand{\Aut}{\textnormal{Aut}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\Hom}{\textnormal{Hom}}
\DeclareMathOperator{\im}{\textnormal{im}}
\newcommand{\coker}{\textnormal{coker} \:}
\newcommand{\id}{\textnormal{id}}

%Diagonal dots looking upwards
\DeclareMathOperator{\rddots}{\cdot^{\cdot^{\cdot}}}

%Special symbol for proofs by contradiction: \lightning
\usepackage{stmaryrd}

%Different numbering for subsections
%\counterwithout{subsection}{section}
%\renewcommand{\thesubsection}{\arabic{subsection}}

%Changing colon into dot for description environment
\renewcommand{\descriptionlabel}[1]{%
  \hspace\labelsep \upshape\bfseries #1.%
}

%Classification theory
\newcommand{\IP}{\textnormal{IP}}
\newcommand{\NIP}{\textnormal{NIP}}
\newcommand{\SOP}{\textnormal{SOP}}
\newcommand{\NSOP}{\textnormal{NSOP}}
\newcommand{\NFSOP}{\textnormal{NFSOP}}
\newcommand{\TP}{\textnormal{TP}}
\newcommand{\NTP}{\textnormal{NTP}}
\newcommand{\FOP}{\textnormal{FOP}}
\newcommand{\NFOP}{\textnormal{NFOP}}
\newcommand{\ATP}{\textnormal{ATP}}
\newcommand{\NATP}{\textnormal{NATP}}
\newcommand{\BTP}{\textnormal{BTP}}
\newcommand{\NBTP}{\textnormal{NBTP}}
\newcommand{\CTP}{\textnormal{CTP}}
\newcommand{\NCTP}{\textnormal{NCTP}}

%Independence relations
\newcommand{\find}{\ind^{\textnormal{f}}}
\newcommand{\dind}{\ind^{\textnormal{d}}}
\newcommand{\iind}{\ind^{\textnormal{i}}}
\newcommand{\uind}{\ind^{\textnormal{u}}}
\newcommand{\hind}{\ind^{\textnormal{h}}}
\newcommand{\kind}{\ind^{\textnormal{K}}}
\newcommand{\aind}{\ind^{\textnormal{a}}}
\newcommand{\istind}{\ind^{\textnormal{ist}}}
\newcommand{\kstind}{\ind^{\textnormal{Kst}}}
\newcommand{\ustind}{\ind^{\textnormal{ust}}}
\newcommand{\cuind}{\ind^{\textnormal{cu}}}
\newcommand{\lind}{\ind^{\textnormal{L}}}
\newcommand{\biind}{\ind^{\textnormal{bi}}}

\newcommand{\sfc}{\textnormal{sfc}}

%For thorns
\usepackage[T1]{fontenc}

%To add notes
\newcommand{\note}[1]{\textcolor{blue}{#1}}

%References
\usepackage[linktocpage, hypertexnames=false]{hyperref}
\hypersetup{
  colorlinks = true, %Colours links instead of ugly boxes
  urlcolor = black, %Colour for external hyperlinks
  linkcolor = black, %Colour of internal links
  citecolor = black %Colour of citations
}
